Uncertainty-Based Ensemble Learning in CMR Semantic Segmentation

Existing methods derive clinical functional metrics from ventricular semantic segmentation in cardiac cine sequences. While performing well on overall segmentation, they struggle with the end slices. To address this, we extract global uncertainty from segmentation variance and use it in our ensemble learning method, Streaming, for classifier weighting, balancing overall and end-slice performance. We introduce the End Coefficient (EC) to quantify end-slice accuracy. Experiments on ACDC and M\&Ms datasets show that our framework achieves near state-of-the-art Dice Similarity Coefficient (DSC) and outperforms all models on end-slice performance, improving patient-specific segmentation accuracy. We open-sourced our code on https://github.com/LEw1sin/Uncertainty-Ensemble.

==> tex/2_Related_Works.tex <==
\section{Related Works}
\subsection{Ensemble Learning}
Müller et al. \cite{muller2022analysis} reviewed three ensemble techniques in medical imaging: \textit{Bagging}, \textit{Stacking}, and \textit{Augmenting}, which are contrasted with our framework Streaming in Fig.~\ref{fig:end-to-end}. \textit{Stacking} trains different networks (i.e. heterogeneous) on the same dataset and pools their outputs, while \textit{Bagging} trains the same type of network (i.e. homogeneous) on different trainsets and aggregates predictions on a shared testset. \textit{Augmenting}, in contrast, uses a single network to process augmented test data, combining outputs via pooling. These methods do not fully exploit deep learning’s end-to-end nature. Our Streaming unifies the dataset and loss function across all components, streamlining training (see \S\ref{sec:end-to-end training}). Unlike traditional pooling methods that aggregate features such as Voting, our approach uses Weighted Average.



\subsection{Uncertainty for Segmentation}
Kendall and Gal \cite{kendall2017uncertainties,li2017dropout, kendall2015bayesian} proposed the use of Bayesian networks to simultaneously manage aleatoric uncertainties caused by data and epistemic uncertainties caused by the network per se. However, these studies focus primarily on integrating uncertainty into the loss function of an existing single segmentation network to optimize its training process. They do not consider leveraging uncertainty to allocate weights among multiple diverse networks to capitalize on their respective strengths within ensemble learning.
